HAO: Hardware-aware neural Architecture Optimization for Efficient Inference

Automatic algorithm-hardware co-design for DNN has shown great success in improving the performance of DNNs on FPGAs. However, this process remains challenging due to the intractable search space of neural network architectures and hardware accelerator implementation. Differing from existing hardware-aware neural architecture search (NAS) algorithms that rely solely on the expensive learning-based approaches, our work incorporates integer programming into the search algorithm to prune the design space. Given a set of hardware resource constraints, our integer programming formulation directly outputs the optimal accelerator configuration for mapping a DNN subgraph that minimizes latency. We use an accuracy predictor for different DNN subgraphs with different quantization schemes and generate accuracy-latency pareto frontiers. With low computational cost, our algorithm can generate quantized networks that achieve state-of-the-art accuracy and hardware performance on Xilinx Zynq (ZU3EG) FPGA for image classification on ImageNet dataset. The solution searched by our algorithm achieves 72.5% top-1 accuracy on ImageNet at framerate 50, which is 60% faster than MnasNet and 135% faster than FBNet with comparable accuracy.

==> 5_ablation_experiments.tex <==
\section{Ablation Study}
\label{sec:ablation}










==> _algo.tex <==
\begin{algorithm}[t]
\DontPrintSemicolon
\caption{Hessian AWare Quantization}
\label{alg:hq}
    \SetAlgoLined
    \KwInput{Block-wise Hessian eigenvalues $\lambda_i$ (computed from~\aref{alg:power_iteration}), and block parameter size $n_i$ 
    for $i=1,\cdots,m$.
    }

    \For(\quad \quad \tcp*[h]{Quantization Precision}){i $=1,2,\ldots, m$}{

        $S_i = \lambda_i/n_i$ \tcp*{See~\eref{eqn:define_S}}
    }
    
    
    Order $S_i$ in descending order and determine relative quantization precision for each block.
    
    Compute $\Delta W_i$ based on~\eref{eqn:quantization_function}.

    \For(\quad \quad \quad \quad \tcp*[h]{Fine-Tuning Order}){i $=1,2,\ldots, m$}{
       $\Omega_i = \lambda_i\|\Delta W_i\|^2$ \tcp*{See~\eref{eqn:define_O}}
    }
    
    Order $\Omega_i$ in descending order and perform block-wise fine-tuning
\end{algorithm}





==> _algo2.tex <==
\begin{algorithm}[t]
\DontPrintSemicolon
\caption{Power Iteration for Hessian Eigenvalue Computation}
\label{alg:power_iteration}
    \SetAlgoLined
    \KwInput{Block Parameter: $W_i$.
    }
    
    Compute the gradient of $W_i$ by backpropagation, \emph{i.e.}, $g_i=\frac{d L}{d W_i}$.
    
    Draw a random vector $v$  (same dimension as $W_i$).
    
    Normalize $v$, $v=\frac{v}{\|v\|}$
    
    \For(\ \ \quad \quad\quad\quad\quad\tcp*[h]{Power Iteration}){i $=1,2,\ldots, n$}{
        Compute $gv = g_i^Tv$ \tcp*{Inner product}
        
        Compute $Hv$ by backpropagation, $Hv = \frac{d(gv)}{dW_i}$ \tcp*{Get Hessian vector product}
        
        Normalize and reset $v$, $v = \frac{Hv}{\|Hv\|}$
    }
\end{algorithm}

==> packages.tex <==

\usepackage{iccv}

\usepackage{soul}
\usepackage[utf8]{inputenc}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{booktabs}


\usepackage{microtype}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{booktabs} %


\input{math_commands.tex}

\usepackage{multirow}
\usepackage{paralist}

\usepackage{booktabs} %
\usepackage{multicol}
\usepackage{diagbox}

\usepackage[ruled,noend]{algorithm2e}
\newcommand{\theHalgorithm}{\arabic{algorithm}}
\newcommand\mycommfont[1]{\scriptsize\ttfamily\textcolor{blue}{#1}}
\SetCommentSty{mycommfont}

\usepackage{here}

\usepackage{amsmath,amssymb,amsfonts,amsbsy,amsfonts,latexsym}
\usepackage{multirow}
\usepackage{makecell}
\usepackage[labelfont=bf,textfont=it,belowskip=0pt,aboveskip=5pt,tableposition=top]{caption}
\usepackage{xcolor}
\usepackage{colortbl}
\let\proof\relax
\let\endproof\relax


\definecolor{colorA}{RGB}{189,201,225}
\definecolor{colorB}{RGB}{103,169,207}
\definecolor{colorC}{RGB}{ 28,144,153}
\definecolor{colorD}{RGB}{  1,108, 89}

\newcolumntype{R}{>{\columncolor{gray!40}}r}
\newcolumntype{L}{>{\columncolor{gray!40}}l}
\newcolumntype{C}{>{\columncolor{gray!40}}c}
\newcommand{\highlightrow}{\rowcolor{orange!20}}




\usepackage{tabularx,colortbl,xcolor}
\usepackage{multirow}
\usepackage[normalem]{ulem}
\useunder{\uline}{\ul}{}

\newcommand\hy{\textrm{-}}

\usepackage{enumitem}

\usepackage{xparse}%

\captionsetup[table]{name=Table}
\DeclareGraphicsExtensions{.pdf,.png}


\SetKwInput{KwInput}{Input}
\newcommand{\pluseq}{\mathrel{+}=}
\newcommand{\asteq}{\mathrel{*}=}
\newcommand{\diveq}{\mathrel{/}=}

\usepackage{longtable}
\usepackage{pgfplots}
